Multiple Imputation Methods under Extreme Values

Missing data are ubiquitous in empirical databases, yet statistical analyses typically require complete data matrices. Multiple imputation offers a principled solution for filling these gaps. This study evaluates the performance of several multiple imputation methods, both in the presence and absence of extreme values, using the MICE package in R. Through Monte Carlo simulations, we generated incomplete data sets with three variables and assessed each imputation method within regression models. The results indicate that the linear regression based imputation method showed the best overall predictive performance (CV-MSE), whereas the sparse model approach was generally less efficient. Our findings underscore the relevance of extreme values when selecting an imputation strategy and highlight sample size, proportion of missingness, presence of extremes, and the type of fitted model as key determinants of performance. Despite its limitations, the study offers practical recommendations for researchers, stressing the need to examine the missingness mechanism and the occurrence of extreme values before choosing an imputation method.

==> figures/figures_n_500.tex <==


% ===== Panel 1: n = 500 =====
\begin{figure}[H]
  \centering
  \adjustbox{width=\textwidth, max height=\textheight, center}{%
    \begin{minipage}{.48\linewidth}
      \includegraphics[page=1 ,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}\\[20pt]
      \includegraphics[page=3 ,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}\\[20pt]
      \includegraphics[page=5 ,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}\\[20pt]
      \includegraphics[page=7 ,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}
    \end{minipage}\hfill
    \begin{minipage}{.48\linewidth}
      \includegraphics[page=2 ,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}\\[20pt]
      \includegraphics[page=4 ,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}\\[20pt]
      \includegraphics[page=6 ,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}\\[20pt]
      \includegraphics[page=8 ,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}
    \end{minipage}%
  }
      \caption{Predictive MSE densities (clean vs contaminated with extremes data), MSE boxplots, and QQ-plots (predicted vs true quantiles of $y$) across six MI methods (T1--T6). For $\boldsymbol{n=500}$, ordered by $P_{\text{ext}}$, and $P_{\text{miss}}$ (panel 1 of 2). Clean data are analyzed with OLS and contaminated data with elastic net. Each subpanel shows the design values ($n$, $P_{\text{ext}}$, $P_{\text{miss}}$, iter, n.sim, and $\rho$).}
      \label{fig:n_500_graficos.1-mesclado-1}%
\end{figure}

% ===== Panel 2: n = 500 =====
\begin{figure}[H]
  \centering
  \adjustbox{width=\textwidth, max height=\textheight, center}{%
    \begin{minipage}{.48\linewidth}
      \includegraphics[page=9 ,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}\\[20pt]
      \includegraphics[page=11,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}
    \end{minipage}\hfill
    \begin{minipage}{.48\linewidth}
      \includegraphics[page=10,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}\\[20pt]
      \includegraphics[page=12,width=\linewidth]{figures/n_500_graficos.1_mesclado.pdf}
    \end{minipage}%
  }
      \caption{Predictive MSE densities (clean vs contaminated with extremes data), MSE boxplots, and QQ-plots (predicted vs true quantiles of $y$) across six MI methods (T1--T6). For $\boldsymbol{n=500}$, ordered by $P_{\text{ext}}$, and $P_{\text{miss}}$ (panel 2 of 2). Clean data are analyzed with OLS and contaminated data with elastic net. Each subpanel shows the design values ($n$, $P_{\text{ext}}$, $P_{\text{miss}}$, iter, n.sim, and $\rho$).}
      \label{fig:n_500_graficos.1-mesclado-2}%
\end{figure}



==> tables/paper.tex <==
% alternative

% ===== Panel 2: n = 500 =====
\begin{figure}[H]
  \centering
  \adjustbox{width=\textwidth, max height=\textheight, center}{%
    \begin{minipage}{.48\linewidth}
      \includegraphics[page=9 ,width=\linewidth]{figures/n_500_graficos.1-mesclado.pdf}\\[20pt]
      \includegraphics[page=11,width=\linewidth]{figures/n_500_graficos.1-mesclado.pdf}
    \end{minipage}\hfill
    \begin{minipage}{.48\linewidth}
      \includegraphics[page=10,width=\linewidth]{figures/n_500_graficos.1-mesclado.pdf}\\[20pt]
      \includegraphics[page=12,width=\linewidth]{figures/n_500_graficos.1-mesclado.pdf}
    \end{minipage}%
  }
      \caption{Predictive MSE densities (clean vs contaminated with extremes data), MSE boxplots, and QQ-plots (predicted vs true quantiles of $y$) across six MI methods (T1--T6). For $\boldsymbol{n=500}$, ordered by $P_{\text{ext}}$, and $P_{\text{miss}}$ (panel 2 of 2). Clean data are analyzed with OLS and contaminated data with elastic net. Each subpanel shows the design values ($n$, $P_{\text{ext}}$, $P_{\text{miss}}$, iter, n.sim, and $\rho$).}
      \label{fig:n_500_graficos.1-mesclado-2}%
\end{figure}

==> tables/tab_n_20_40.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% n_20_40 - table 1
\begin{table}[H]
\centering
\caption{Bias, RMSE, and 95\% coverage for $(\beta_0,\beta_1,\beta_2)$ under clean data with OLS and data with extreme values using elastic net (EN), for $\boldsymbol{n=20}$ (left) and $\boldsymbol{n=40}$ (right). Entries are reported as min--max within each missingness block (low: $P_{\text{miss}}\in\{0.05,0.10\}$; and high: $P_{\text{miss}}\in\{0.25,0.30\}$). Ranges further aggregate over all design combinations $P_{\text{ext}}\in\{0.03,0.05,0.10,0.15,0.30\}$, n.sim $\in\{50,300,1000\}$, $\text{iter}\in\{5,10\}$, and $\rho\in\{0,0.6\}$. MI methods are grouped as parametric (T1--T3: \texttt{norm.predict}, \texttt{lasso.select.norm}, \texttt{norm.boot}), donor/ML (T4--T6: \texttt{pmm}, \texttt{rf}, \texttt{midastouch}), and the combined set (T1--T6). Coverage is the proportion of 95\% intervals containing the true coefficient}
\label{tab:resumo_20_40_1}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l l c c c c c c @{}}
\toprule
\multicolumn{2}{c}{} & \multicolumn{3}{c}{\textbf{n = 20}} & \multicolumn{3}{c}{\textbf{n = 40}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
MI & Metric & $\beta_0$ & $\beta_1$ & $\beta_2$ & $\beta_0$ & $\beta_1$ & $\beta_2$ \\
\midrule
\multicolumn{8}{l}{\textbf{Linear regression (OLS):} low missing-data proportion (5\% and 10\%)}\\ 
T1--T3 & Bias & [-0.424 , -0.097] & [-0.043 , -0.007] & [0.038 , 0.158] & [1.940 , 2.503] & [-0.203 , -0.131] & [-0.226 , -0.121] \\
T1--T3 & RMSE & [0.315 , 0.539] & [0.023 , 0.097] & [0.059 , 0.246] & [1.963 , 2.526] & [0.135 , 0.205] & [0.127 , 0.228] \\
T1--T3 & Coverage & [1.000 , 1.000] & [0.990 , 1.000] & [0.980 , 1.000] & [0.680 , 0.980] & [0.620 , 1.000] & [1.000 , 1.000] \\
T4--T6 & Bias & [-0.286 , -0.023] & [-0.025 , 0.002] & [0.012 , 0.086] & [1.886 , 2.574] & [-0.193 , -0.102] & [-0.266 , -0.167] \\
T4--T6 & RMSE & [0.290 , 0.478] & [0.026 , 0.097] & [0.050 , 0.205] & [1.931 , 2.619] & [0.121 , 0.197] & [0.173 , 0.276] \\
T4--T6 & Coverage & [1.000 , 1.000] & [0.993 , 1.000] & [0.990 , 1.000] & [0.720 , 0.980] & [0.880 , 1.000] & [1.000 , 1.000] \\
T1--T6 & Bias & [-0.424 , -0.023] & [-0.043 , 0.002] & [0.012 , 0.158] & [1.886 , 2.574] & [-0.203 , -0.102] & [-0.266 , -0.121] \\
T1--T6 & RMSE & [0.290 , 0.539] & [0.023 , 0.097] & [0.050 , 0.246] & [1.931 , 2.619] & [0.121 , 0.205] & [0.127 , 0.276] \\
T1--T6 & Coverage & [1.000 , 1.000] & [0.990 , 1.000] & [0.980 , 1.000] & [0.680 , 0.980] & [0.620 , 1.000] & [1.000 , 1.000] \\
\addlinespace[3pt]
\cmidrule(lr){1-8}
\multicolumn{8}{l}{\textbf{Linear regression (OLS):} high missing-data proportion (25\% and 30\%)}\\ 
T1--T3 & Bias & [-0.875 , 0.294] & [-0.113 , -0.051] & [0.085 , 0.331] & [1.858 , 2.766] & [-0.232 , -0.141] & [-0.228 , 0.008] \\
T1--T3 & RMSE & [0.726 , 1.151] & [0.145 , 0.214] & [0.303 , 0.470] & [1.927 , 2.830] & [0.154 , 0.241] & [0.065 , 0.245] \\
T1--T3 & Coverage & [0.980 , 1.000] & [0.903 , 0.987] & [0.799 , 0.973] & [0.640 , 0.820] & [0.320 , 1.000] & [1.000 , 1.000] \\
T4--T6 & Bias & [-0.406 , 0.191] & [-0.033 , 0.003] & [-0.016 , 0.117] & [1.863 , 3.087] & [-0.206 , -0.074] & [-0.365 , -0.161] \\
T4--T6 & RMSE & [0.643 , 0.837] & [0.116 , 0.164] & [0.238 , 0.353] & [1.946 , 3.163] & [0.110 , 0.217] & [0.182 , 0.383] \\
T4--T6 & Coverage & [1.000 , 1.000] & [0.980 , 1.000] & [0.940 , 1.000] & [0.720 , 0.940] & [0.860 , 1.000] & [1.000 , 1.000] \\
T1--T6 & Bias & [-0.875 , 0.294] & [-0.113 , 0.003] & [-0.016 , 0.331] & [1.858 , 3.087] & [-0.232 , -0.074] & [-0.365 , 0.008] \\
T1--T6 & RMSE & [0.643 , 1.151] & [0.116 , 0.214] & [0.238 , 0.470] & [1.927 , 3.163] & [0.110 , 0.241] & [0.065 , 0.383] \\
T1--T6 & Coverage & [0.980 , 1.000] & [0.903 , 1.000] & [0.799 , 1.000] & [0.640 , 0.940] & [0.320 , 1.000] & [1.000 , 1.000] \\
\addlinespace[3pt]
\cmidrule(lr){1-8}
\multicolumn{8}{l}{\textbf{Sparse regression (EN)}: low missing-data proportion (5\% and 10\%)} \\ 
T1--T3 & Bias & [0.888 , 1.662] & [-0.356 , -0.225] & [0.197 , 0.399] & [2.235 , 3.652] & [-0.239 , -0.082] & [-0.433 , -0.245] \\
T1--T3 & RMSE & [0.932 , 1.815] & [0.229 , 0.361] & [0.201 , 0.405] & [2.243 , 3.669] & [0.092 , 0.241] & [0.248 , 0.438] \\
T1--T3 & Coverage & [0.900 , 1.000] & [0.860 , 1.000] & [0.902 , 1.000] & [0.000 , 0.340] & [0.040 , 1.000] & [0.460 , 1.000] \\
T4--T6 & Bias & [0.081 , 1.382] & [-0.264 , -0.047] & [-0.007 , 0.237] & [2.197 , 3.581] & [-0.221 , -0.061] & [-0.454 , -0.298] \\
T4--T6 & RMSE & [0.558 , 1.582] & [0.149 , 0.275] & [0.115 , 0.283] & [2.212 , 3.617] & [0.079 , 0.226] & [0.303 , 0.460] \\
T4--T6 & Coverage & [0.950 , 1.000] & [0.940 , 1.000] & [0.950 , 1.000] & [0.000 , 0.320] & [0.460 , 1.000] & [0.480 , 1.000] \\
T1--T6 & Bias & [0.081 , 1.662] & [-0.356 , -0.047] & [-0.007 , 0.399] & [2.197 , 3.652] & [-0.239 , -0.061] & [-0.454 , -0.245] \\
T1--T6 & RMSE & [0.558 , 1.815] & [0.149 , 0.361] & [0.115 , 0.405] & [2.212 , 3.669] & [0.079 , 0.241] & [0.248 , 0.460] \\
T1--T6 & Coverage & [0.900 , 1.000] & [0.860 , 1.000] & [0.902 , 1.000] & [0.000 , 0.340] & [0.040 , 1.000] & [0.460 , 1.000] \\
\addlinespace[3pt]
\cmidrule(lr){1-8}
\multicolumn{8}{l}{\textbf{Sparse regression (EN)}: high missing-data proportion (25\% and 30\%)} \\ 
T1--T3 & Bias & [0.983 , 1.809] & [-0.396 , -0.241] & [0.211 , 0.423] & [2.037 , 3.599] & [-0.262 , -0.068] & [-0.448 , -0.090] \\
T1--T3 & RMSE & [1.158 , 2.124] & [0.261 , 0.429] & [0.242 , 0.459] & [2.095 , 3.661] & [0.102 , 0.272] & [0.151 , 0.465] \\
T1--T3 & Coverage & [0.740 , 1.000] & [0.428 , 1.000] & [0.660 , 1.000] & [0.060 , 0.640] & [0.100 , 1.000] & [0.720 , 1.000] \\
T4--T6 & Bias & [-0.612 , 0.867] & [-0.197 , 0.102] & [-0.228 , 0.191] & [1.833 , 3.456] & [-0.193 , 0.006] & [-0.520 , -0.314] \\
T4--T6 & RMSE & [1.229 , 1.707] & [0.144 , 0.259] & [0.124 , 0.276] & [1.903 , 3.573] & [0.079 , 0.213] & [0.329 , 0.534] \\
T4--T6 & Coverage & [0.978 , 1.000] & [0.980 , 1.000] & [0.980 , 1.000] & [0.220 , 0.720] & [0.720 , 1.000] & [0.600 , 0.900] \\
T1--T6 & Bias & [-0.612 , 1.809] & [-0.396 , 0.102] & [-0.228 , 0.423] & [1.833 , 3.599] & [-0.262 , 0.006] & [-0.520 , -0.090] \\
T1--T6 & RMSE & [1.158 , 2.124] & [0.144 , 0.429] & [0.124 , 0.459] & [1.903 , 3.661] & [0.079 , 0.272] & [0.151 , 0.534] \\
T1--T6 & Coverage & [0.740 , 1.000] & [0.428 , 1.000] & [0.660 , 1.000] & [0.060 , 0.720] & [0.100 , 1.000] & [0.600 , 1.000] \\
\addlinespace[3pt]
\bottomrule
\end{tabular*}
\endgroup
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% n_20_40 - table 2
\begin{table}[H]
\centering
% ---------- TABLE 2 ----------
\caption{Out-of-sample predictive error summaries (CV–MSE) by MI method for $\boldsymbol{n=20}$ (left) and $\boldsymbol{n=40}$ (right), stratified by model (OLS for clean data; elastic net (EN) for contaminated data) and by missingness blocks (low: $P_{\text{miss}}\in\{0.05,0.10\}$; and high: $P_{\text{miss}}\in\{0.25,0.30\}$). For each method it is reported the min-max of the MSE: mean $\overline{X}$, variance $\sigma^2$, and median $Q_{50}$ across the corresponding design cells. Ranges further aggregate over all design combinations $P_{\text{ext}}\in\{0.03,0.05,0.10,0.15,0.30\}$, $\text{n.sim}\in\{50,300,1000\}$, $\text{iter}\in\{5,10\}$, and $\rho\in\{0,0.6\}$}
\label{tab:resumo_20_40_2}
\begingroup
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l c c c c c c @{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{n = 20}} & \multicolumn{3}{c}{\textbf{n = 40}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
MI & $\overline{X}$ & $\sigma^2$ & $Q_{50}$ & $\overline{X}$ & $\sigma^2$ & $Q_{50}$ \\
\midrule
\multicolumn{7}{l}{\textbf{Linear regression (OLS):} low missing-data proportion (5\% and 10\%)} \\
T1 & [2.283 , 2.524] & [0.236 , 0.461] & [2.206 , 2.450] & [2.077 , 2.207] & [0.020 , 0.050] & [2.110 , 2.241] \\
T2 & [2.441 , 2.690] & [0.200 , 0.413] & [2.407 , 2.576] & [2.242 , 2.271] & [0.019 , 0.057] & [2.265 , 2.285] \\
T3 & [2.399 , 2.620] & [0.196 , 0.369] & [2.336 , 2.500] & [2.236 , 2.275] & [0.018 , 0.061] & [2.228 , 2.280] \\
T4 & [2.473 , 2.693] & [0.240 , 0.429] & [2.433 , 2.578] & [2.273 , 2.357] & [0.023 , 0.125] & [2.260 , 2.346] \\
T5 & [2.611 , 2.909] & [0.173 , 0.736] & [2.553 , 2.766] & [2.351 , 2.560] & [0.053 , 0.213] & [2.312 , 2.479] \\
T6 & [2.432 , 2.672] & [0.226 , 0.465] & [2.399 , 2.547] & [2.273 , 2.337] & [0.024 , 0.112] & [2.253 , 2.354] \\
\addlinespace[4pt]
\cmidrule(lr){1-7}
\multicolumn{7}{l}{\textbf{Linear regression (OLS):} high missing-data proportion (25\% and 30\%)} \\
T1 & [1.912 , 2.166] & [0.252 , 0.496] & [1.956 , 2.081] & [1.725 , 1.819] & [0.093 , 0.121] & [1.757 , 1.858] \\
T2 & [2.484 , 2.628] & [0.292 , 0.419] & [2.470 , 2.666] & [2.256 , 2.334] & [0.123 , 0.176] & [2.275 , 2.351] \\
T3 & [2.296 , 2.494] & [0.265 , 0.415] & [2.390 , 2.491] & [2.236 , 2.261] & [0.158 , 0.193] & [2.230 , 2.297] \\
T4 & [2.635 , 2.712] & [0.246 , 0.428] & [2.631 , 2.737] & [2.516 , 2.605] & [0.274 , 0.312] & [2.480 , 2.589] \\
T5 & [3.015 , 3.355] & [0.204 , 0.524] & [3.070 , 3.390] & [2.890 , 3.201] & [0.248 , 0.403] & [2.878 , 3.140] \\
T6 & [2.506 , 2.616] & [0.235 , 0.501] & [2.530 , 2.666] & [2.434 , 2.470] & [0.221 , 0.340] & [2.364 , 2.435] \\
\addlinespace[4pt]
\cmidrule(lr){1-7}
\multicolumn{7}{l}{\textbf{Sparse regression (EN)}: low missing-data proportion (5\% and 10\%)} \\
T1 & [1.441 , 1.995] & [0.038 , 0.095] & [1.438 , 1.943] & [2.505 , 2.867] & [0.032 , 0.091] & [2.574 , 2.867] \\
T2 & [1.577 , 2.118] & [0.046 , 0.162] & [1.566 , 2.072] & [2.687 , 2.923] & [0.033 , 0.113] & [2.716 , 2.964] \\
T3 & [1.558 , 2.083] & [0.045 , 0.142] & [1.549 , 2.056] & [2.704 , 2.911] & [0.035 , 0.116] & [2.715 , 2.948] \\
T4 & [1.906 , 2.553] & [0.175 , 1.002] & [1.675 , 2.274] & [2.771 , 2.925] & [0.057 , 0.199] & [2.750 , 2.944] \\
T5 & [2.275 , 3.103] & [0.302 , 1.721] & [1.935 , 2.740] & [2.822 , 3.045] & [0.059 , 0.246] & [2.776 , 3.042] \\
T6 & [1.846 , 2.380] & [0.150 , 0.877] & [1.618 , 2.180] & [2.735 , 2.914] & [0.056 , 0.160] & [2.722 , 2.943] \\
\addlinespace[4pt]
\cmidrule(lr){1-7}
\multicolumn{7}{l}{\textbf{Sparse regression (EN)}: high missing-data proportion (25\% and 30\%)} \\
T1 & [1.180 , 1.635] & [0.072 , 0.165] & [1.146 , 1.616] & [2.162 , 2.529] & [0.136 , 0.155] & [2.177 , 2.558] \\
T2 & [1.780 , 2.403] & [0.174 , 0.361] & [1.698 , 2.361] & [2.734 , 2.948] & [0.134 , 0.217] & [2.779 , 2.969] \\
T3 & [1.703 , 2.270] & [0.139 , 0.317] & [1.655 , 2.179] & [2.710 , 2.896] & [0.137 , 0.201] & [2.704 , 2.878] \\
T4 & [3.258 , 3.703] & [1.237 , 1.734] & [2.974 , 3.524] & [2.961 , 3.252] & [0.108 , 0.334] & [3.009 , 3.264] \\
T5 & [4.243 , 5.068] & [1.351 , 2.908] & [3.928 , 5.008] & [3.153 , 3.560] & [0.123 , 0.505] & [3.136 , 3.590] \\
T6 & [2.847 , 3.197] & [1.182 , 2.461] & [2.572 , 2.891] & [2.857 , 3.079] & [0.144 , 0.322] & [2.919 , 2.997] \\
\addlinespace[4pt]
\bottomrule
\end{tabular*}
\endgroup
\end{table}



==> tables/tab_n_500.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% n_500 - table 1 (HEADER COM n = 500)
\begin{table}[htbp]
\centering
\caption{Bias, RMSE, and 95\% coverage for $(\beta_0,\beta_1,\beta_2)$ under clean data with OLS and data with extreme values using elastic net (EN), for $\boldsymbol{n=20}$ (left) and $\boldsymbol{n=40}$ (right). Entries are reported as min--max within each missingness block (low: $P_{\text{miss}}\in\{0.05,0.10\}$; and high: $P_{\text{miss}}\in\{0.25,0.30\}$). Ranges further aggregate over all design combinations $P_{\text{ext}}\in\{0.03,0.05,0.10,0.15,0.30\}$, n.sim $\in\{50,300,1000\}$, $\text{iter}\in\{5,10\}$, and $\rho\in\{0,0.6\}$. MI methods are grouped as parametric (T1--T3: \texttt{norm.predict}, \texttt{lasso.select.norm}, \texttt{norm.boot}), donor/ML (T4--T6: \texttt{pmm}, \texttt{rf}, \texttt{midastouch}), and the combined set (T1--T6). Coverage is the proportion of 95\% intervals containing the true coefficient}
\label{tab:resumo_500_1}
\begingroup
\scriptsize
\begin{tabular*}{0.7\textwidth}{@{\extracolsep{\fill}} l l c c c @{}}
\toprule
\multicolumn{2}{c}{} & \multicolumn{3}{c}{\textbf{n = 500}} \\
\cmidrule(lr){3-5}
Case & Metrics & $\beta_0$ & $\beta_1$ & $\beta_2$ \\
\midrule

% ---- OLS ; Pmiss 0.05/0.10 ----
\multicolumn{5}{@{}l@{}}{\textbf{Linear regression (OLS)} \quad \textit{\( P_{\text{miss}} \in \{0.05, 0.10\} \)}} \\ 
T1--T3 & Bias & [0.057 , 0.177] & [-0.007 , 0.018] & [-0.058 , 0.013] \\
T1--T3 & RMSE & [0.109 , 0.206] & [0.008 , 0.020] & [0.017 , 0.059] \\
T1--T3 & Coverage & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] \\
T4--T6 & Bias & [0.158 , 0.188] & [0.016 , 0.019] & [-0.064 , -0.053] \\
T4--T6 & RMSE & [0.179 , 0.215] & [0.018 , 0.022] & [0.055 , 0.066] \\
T4--T6 & Coverage & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] \\
T1--T6 & Bias & [0.057 , 0.188] & [-0.007 , 0.019] & [-0.064 , 0.013] \\
T1--T6 & RMSE & [0.109 , 0.215] & [0.008 , 0.022] & [0.017 , 0.066] \\
T1--T6 & Coverage & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] \\

\addlinespace[2pt]
\cmidrule(lr){1-5}

% ---- OLS ; Pmiss 0.25/0.30 ----
\multicolumn{5}{@{}l@{}}{\textbf{Linear regression (OLS)} \quad \textit{\( P_{\text{miss}} \in \{0.25, 0.30\} \)}} \\ 
T1--T3 & Bias & [-0.200 , 0.206] & [-0.064 , 0.017] & [-0.061 , 0.174] \\
T1--T3 & RMSE & [0.251 , 0.294] & [0.024 , 0.067] & [0.060 , 0.176] \\
T1--T3 & Coverage & [0.960 , 1.000] & [0.580 , 1.000] & [0.000 , 1.000] \\
T4--T6 & Bias & [0.138 , 0.227] & [0.017 , 0.026] & [-0.083 , -0.055] \\
T4--T6 & RMSE & [0.222 , 0.299] & [0.025 , 0.033] & [0.060 , 0.088] \\
T4--T6 & Coverage & [0.997 , 1.000] & [0.980 , 1.000] & [0.960 , 1.000] \\
T1--T6 & Bias & [-0.200 , 0.227] & [-0.064 , 0.026] & [-0.083 , 0.174] \\
T1--T6 & RMSE & [0.222 , 0.299] & [0.024 , 0.067] & [0.060 , 0.176] \\
T1--T6 & Coverage & [0.960 , 1.000] & [0.580 , 1.000] & [0.000 , 1.000] \\

\addlinespace[2pt]
\cmidrule(lr){1-5}

% ---- EN ; Pmiss 0.05/0.10 ----
\multicolumn{5}{@{}l@{}}{\textbf{Sparse regression (elastic net)} \quad \textit{\( P_{\text{miss}} \in \{0.05, 0.10\} \)}} \\ 
T1--T3 & Bias & [0.076 , 0.270] & [-0.108 , -0.060] & [0.080 , 0.162] \\
T1--T3 & RMSE & [0.087 , 0.285] & [0.061 , 0.108] & [0.081 , 0.163] \\
T1--T3 & Coverage & [1.000 , 1.000] & [0.000 , 0.860] & [0.000 , 1.000] \\
T4--T6 & Bias & [0.082 , 0.289] & [-0.083 , -0.056] & [0.076 , 0.109] \\
T4--T6 & RMSE & [0.092 , 0.300] & [0.057 , 0.084] & [0.076 , 0.110] \\
T4--T6 & Coverage & [0.997 , 1.000] & [0.000 , 0.900] & [0.300 , 1.000] \\
T1--T6 & Bias & [0.076 , 0.289] & [-0.108 , -0.056] & [0.076 , 0.162] \\
T1--T6 & RMSE & [0.087 , 0.300] & [0.057 , 0.108] & [0.076 , 0.163] \\
T1--T6 & Coverage & [0.997 , 1.000] & [0.000 , 0.900] & [0.000 , 1.000] \\

\addlinespace[2pt]
\cmidrule(lr){1-5}

% ---- EN ; Pmiss 0.25/0.30 ----
\multicolumn{5}{@{}l@{}}{\textbf{Sparse regression (elastic net)} \quad \textit{\( P_{\text{miss}} \in \{0.25, 0.30\} \)}} \\ 
T1--T3 & Bias & [0.007 , 0.294] & [-0.168 , -0.066] & [0.076 , 0.284] \\
T1--T3 & RMSE & [0.150 , 0.334] & [0.068 , 0.169] & [0.079 , 0.285] \\
T1--T3 & Coverage & [0.912 , 1.000] & [0.000 , 0.840] & [0.000 , 0.980] \\
T4--T6 & Bias & [0.206 , 0.367] & [-0.086 , -0.055] & [0.046 , 0.112] \\
T4--T6 & RMSE & [0.236 , 0.385] & [0.058 , 0.088] & [0.050 , 0.115] \\
T4--T6 & Coverage & [0.920 , 1.000] & [0.272 , 0.940] & [0.420 , 1.000] \\
T1--T6 & Bias & [0.007 , 0.367] & [-0.168 , -0.055] & [0.046 , 0.284] \\
T1--T6 & RMSE & [0.150 , 0.385] & [0.058 , 0.169] & [0.050 , 0.285] \\
T1--T6 & Coverage & [0.912 , 1.000] & [0.000 , 0.940] & [0.000 , 1.000] \\

\bottomrule
\end{tabular*}
\endgroup
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% n_500 - table 2 (HEADER COM n = 500)
\begin{table}[H]
\centering
\caption{Out-of-sample predictive error summaries (CV–MSE) by MI method for $\boldsymbol{n = 500}$, stratified by model (OLS for clean data; elastic net (EN) for contaminated data) and by missingness blocks (low: $P_{\text{miss}}\in\{0.05,0.10\}$; and high: $P_{\text{miss}}\in\{0.25,0.30\}$). For each method it is reported the min-max of the MSE: mean $\overline{X}$, variance $\sigma^2$, and median $Q_{50}$ across the corresponding design cells. Ranges further aggregate over all design combinations $P_{\text{ext}}\in\{0.03,0.05,0.10,0.15,0.30\}$, $\text{n.sim}\in\{50,300,1000\}$, $\text{iter}\in\{5,10\}$, and $\rho\in\{0,0.6\}$}
\label{tab:resumo_500_2}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.06}

% ajuste 0.64\textwidth para casar com o comprimento do texto do \multicolumn
\begin{tabular*}{0.64\textwidth}{@{}p{11mm}*{3}{>{\centering\arraybackslash}p{\dimexpr(0.64\textwidth-11mm)/3\relax}}@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{n = 500}} \\
\cmidrule(lr){2-4}
MI & $\overline{X}$ & $\sigma^2$ & $Q_{50}$ \\
\midrule

% ---- OLS ; Pmiss 0.05/0.10 ----
\multicolumn{4}{l}{\textbf{Linear regression (OLS):} low missing-data proportion (5\% and 10\%)} \\
T1 & [2.081 , 2.153] & [0.001 , 0.002] & [2.079 , 2.154] \\
T2 & [2.208 , 2.222] & [0.001 , 0.003] & [2.202 , 2.222] \\
T3 & [2.209 , 2.220] & [0.001 , 0.003] & [2.206 , 2.221] \\
T4 & [2.211 , 2.224] & [0.001 , 0.003] & [2.204 , 2.226] \\
T5 & [2.224 , 2.255] & [0.001 , 0.003] & [2.221 , 2.255] \\
T6 & [2.207 , 2.225] & [0.001 , 0.003] & [2.211 , 2.226] \\

\addlinespace[4pt]
\cmidrule(lr){1-4}

% ---- OLS ; Pmiss 0.25/0.30 ----
\multicolumn{4}{l}{\textbf{Linear regression (OLS):} high missing-data proportion (25\% and 30\%)} \\
T1 & [1.784 , 1.797] & [0.005 , 0.008] & [1.786 , 1.796] \\
T2 & [2.211 , 2.230] & [0.007 , 0.011] & [2.213 , 2.229] \\
T3 & [2.208 , 2.221] & [0.007 , 0.012] & [2.194 , 2.220] \\
T4 & [2.221 , 2.235] & [0.005 , 0.011] & [2.226 , 2.246] \\
T5 & [2.323 , 2.335] & [0.006 , 0.010] & [2.314 , 2.340] \\
T6 & [2.221 , 2.237] & [0.006 , 0.012] & [2.232 , 2.235] \\

\addlinespace[4pt]
\cmidrule(lr){1-4}

% ---- EN ; Pmiss 0.05/0.10 ----
\multicolumn{4}{l}{\textbf{Sparse regression (EN)}: low missing-data proportion (5\% and 10\%)} \\
T1 & [1.342 , 2.080] & [0.001 , 0.003] & [1.343 , 2.083] \\
T2 & [1.443 , 2.154] & [0.001 , 0.003] & [1.446 , 2.158] \\
T3 & [1.442 , 2.151] & [0.001 , 0.003] & [1.444 , 2.149] \\
T4 & [1.450 , 2.155] & [0.001 , 0.004] & [1.450 , 2.160] \\
T5 & [1.499 , 2.203] & [0.001 , 0.004] & [1.491 , 2.213] \\
T6 & [1.453 , 2.150] & [0.001 , 0.004] & [1.454 , 2.156] \\

\addlinespace[4pt]
\cmidrule(lr){1-4}

% ---- EN ; Pmiss 0.25/0.30 ----
\multicolumn{4}{l}{\textbf{Sparse regression (EN)}: high missing-data proportion (25\% and 30\%)} \\
T1 & [1.494 , 1.694] & [0.005 , 0.006] & [1.495 , 1.694] \\
T2 & [1.939 , 2.172] & [0.006 , 0.009] & [1.940 , 2.165] \\
T3 & [1.924 , 2.153] & [0.007 , 0.009] & [1.923 , 2.143] \\
T4 & [1.931 , 2.160] & [0.007 , 0.010] & [1.934 , 2.151] \\
T5 & [2.124 , 2.354] & [0.008 , 0.015] & [2.122 , 2.340] \\
T6 & [1.936 , 2.147] & [0.008 , 0.009] & [1.931 , 2.149] \\

\addlinespace[4pt]
\bottomrule
\end{tabular*}
\endgroup
\end{table}


==> tables/tab_n_80_200.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%% tab_n_80_200 - table 1
\begin{table}[H]
\centering
\caption{Bias, RMSE, and 95\% coverage for $(\beta_0,\beta_1,\beta_2)$ under clean data with OLS and data with extreme values using elastic net (EN), for $\boldsymbol{n=80}$ (left) and $\boldsymbol{n=200}$ (right). Entries are reported as min--max within each missingness block (low: $P_{\text{miss}}\in\{0.05,0.10\}$; and high: $P_{\text{miss}}\in\{0.25,0.30\}$). Ranges further aggregate over all design combinations $P_{\text{ext}}\in\{0.03,0.05,0.10,0.15,0.30\}$, n.sim $\in\{50,300,1000\}$, $\text{iter}\in\{5,10\}$, and $\rho\in\{0,0.6\}$. MI methods are grouped as parametric (T1--T3: \texttt{norm.predict}, \texttt{lasso.select.norm}, \texttt{norm.boot}), donor/ML (T4--T6: \texttt{pmm}, \texttt{rf}, \texttt{midastouch}), and the combined set (T1--T6). Coverage is the proportion of 95\% intervals containing the true coefficient}
\label{tab:resumo_80_200_1}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l l c c c c c c @{}}
\toprule
\multicolumn{2}{c}{} & \multicolumn{3}{c}{\textbf{n = 80}} & \multicolumn{3}{c}{\textbf{n = 200}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
Case & Metrics & $\beta_0$ & $\beta_1$ & $\beta_2$ & $\beta_0$ & $\beta_1$ & $\beta_2$ \\
\midrule
\multicolumn{8}{l}{\textbf{Linear regression (OLS):} low missing-data proportion (5\% and 10\%)} \\ 
T1--T3 & Bias & [0.147 , 0.425] & [0.021 , 0.037] & [-0.199 , -0.115] & [-0.268 , 0.034] & [-0.018 , 0.003] & [0.002 , 0.067] \\
T1--T3 & RMSE & [0.301 , 0.487] & [0.030 , 0.046] & [0.124 , 0.203] & [0.128 , 0.350] & [0.011 , 0.022] & [0.015 , 0.071] \\
T1--T3 & Coverage & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] \\
T4--T6 & Bias & [0.359 , 0.475] & [0.026 , 0.037] & [-0.213 , -0.183] & [-0.047 , 0.144] & [-0.009 , 0.001] & [-0.010 , 0.010] \\
T4--T6 & RMSE & [0.411 , 0.533] & [0.037 , 0.045] & [0.189 , 0.218] & [0.127 , 0.295] & [0.010 , 0.022] & [0.014 , 0.028] \\
T4--T6 & Coverage & [1.000 , 1.000] & [1.000 , 1.000] & [0.980 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] \\
T1--T6 & Bias & [0.147 , 0.475] & [0.021 , 0.037] & [-0.213 , -0.115] & [-0.268 , 0.144] & [-0.018 , 0.003] & [-0.010 , 0.067] \\
T1--T6 & RMSE & [0.301 , 0.533] & [0.030 , 0.046] & [0.124 , 0.218] & [0.127 , 0.350] & [0.010 , 0.022] & [0.014 , 0.071] \\
T1--T6 & Coverage & [1.000 , 1.000] & [1.000 , 1.000] & [0.980 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] \\
\addlinespace[3pt]
\cmidrule(lr){1-8}
\multicolumn{8}{l}{\textbf{Linear regression (OLS):} high missing-data proportion (25\% and 30\%)} \\ 
T1--T3 & Bias & [-0.368 , 0.444] & [-0.007 , 0.039] & [-0.207 , 0.047] & [-0.872 , -0.004] & [-0.045 , 0.018] & [-0.001 , 0.196] \\
T1--T3 & RMSE & [0.485 , 0.683] & [0.041 , 0.059] & [0.075 , 0.230] & [0.336 , 0.990] & [0.029 , 0.055] & [0.035 , 0.201] \\
T1--T3 & Coverage & [0.980 , 1.000] & [0.993 , 1.000] & [0.900 , 1.000] & [0.680 , 1.000] & [0.940 , 1.000] & [0.100 , 1.000] \\
T4--T6 & Bias & [0.354 , 0.632] & [0.032 , 0.049] & [-0.259 , -0.188] & [-0.175 , 0.473] & [-0.020 , 0.015] & [-0.051 , 0.015] \\
T4--T6 & RMSE & [0.527 , 0.796] & [0.050 , 0.062] & [0.209 , 0.280] & [0.385 , 0.656] & [0.033 , 0.042] & [0.037 , 0.064] \\
T4--T6 & Coverage & [1.000 , 1.000] & [1.000 , 1.000] & [0.840 , 0.960] & [1.000 , 1.000] & [1.000 , 1.000] & [1.000 , 1.000] \\
T1--T6 & Bias & [-0.368 , 0.632] & [-0.007 , 0.049] & [-0.259 , 0.047] & [-0.872 , 0.473] & [-0.045 , 0.018] & [-0.051 , 0.196] \\
T1--T6 & RMSE & [0.485 , 0.796] & [0.041 , 0.062] & [0.075 , 0.280] & [0.336 , 0.990] & [0.029 , 0.055] & [0.035 , 0.201] \\
T1--T6 & Coverage & [0.980 , 1.000] & [0.993 , 1.000] & [0.840 , 1.000] & [0.680 , 1.000] & [0.940 , 1.000] & [0.100 , 1.000] \\
\addlinespace[3pt]
\cmidrule(lr){1-8}
\multicolumn{8}{l}{\textbf{Sparse regression (EN)}: low missing-data proportion (5\% and 10\%)} \\ 
T1--T3 & Bias & [-0.285 , 0.047] & [0.083 , 0.136] & [-0.227 , -0.144] & [0.663 , 1.738] & [-0.090 , 0.011] & [-0.144 , 0.007] \\
T1--T3 & RMSE & [0.113 , 0.346] & [0.086 , 0.139] & [0.145 , 0.228] & [0.666 , 1.743] & [0.010 , 0.091] & [0.017 , 0.145] \\
T1--T3 & Coverage & [1.000 , 1.000] & [0.980 , 1.000] & [0.188 , 1.000] & [0.000 , 1.000] & [0.560 , 1.000] & [0.100 , 1.000] \\
T4--T6 & Bias & [-0.352 , -0.010] & [0.109 , 0.155] & [-0.252 , -0.196] & [0.682 , 1.830] & [-0.090 , 0.011] & [-0.151 , -0.058] \\
T4--T6 & RMSE & [0.100 , 0.437] & [0.112 , 0.158] & [0.197 , 0.255] & [0.684 , 1.833] & [0.013 , 0.090] & [0.061 , 0.152] \\
T4--T6 & Coverage & [1.000 , 1.000] & [0.920 , 1.000] & [0.170 , 1.000] & [0.000 , 1.000] & [0.800 , 1.000] & [0.040 , 1.000] \\
T1--T6 & Bias & [-0.352 , 0.047] & [0.083 , 0.155] & [-0.252 , -0.144] & [0.663 , 1.830] & [-0.090 , 0.011] & [-0.151 , 0.007] \\
T1--T6 & RMSE & [0.100 , 0.437] & [0.086 , 0.158] & [0.145 , 0.255] & [0.666 , 1.833] & [0.010 , 0.091] & [0.017 , 0.152] \\
T1--T6 & Coverage & [1.000 , 1.000] & [0.920 , 1.000] & [0.170 , 1.000] & [0.000 , 1.000] & [0.560 , 1.000] & [0.040 , 1.000] \\
\addlinespace[3pt]
\cmidrule(lr){1-8}
\multicolumn{8}{l}{\textbf{Sparse regression (EN)}: high missing-data proportion (25\% and 30\%)} \\ 
T1--T3 & Bias & [-0.506 , 0.039] & [0.037 , 0.138] & [-0.221 , -0.014] & [0.604 , 1.717] & [-0.122 , 0.013] & [-0.148 , 0.151] \\
T1--T3 & RMSE & [0.261 , 0.707] & [0.057 , 0.148] & [0.055 , 0.228] & [0.665 , 1.733] & [0.027 , 0.125] & [0.037 , 0.155] \\
T1--T3 & Coverage & [0.980 , 1.000] & [0.880 , 1.000] & [0.673 , 1.000] & [0.000 , 0.900] & [0.000 , 1.000] & [0.380 , 1.000] \\
T4--T6 & Bias & [-0.707 , -0.016] & [0.108 , 0.215] & [-0.334 , -0.199] & [0.715 , 1.976] & [-0.106 , 0.018] & [-0.175 , -0.066] \\
T4--T6 & RMSE & [0.233 , 0.939] & [0.116 , 0.228] & [0.207 , 0.342] & [0.751 , 1.983] & [0.024 , 0.111] & [0.076 , 0.177] \\
T4--T6 & Coverage & [0.920 , 1.000] & [0.660 , 0.967] & [0.380 , 0.920] & [0.000 , 0.940] & [0.500 , 1.000] & [0.180 , 1.000] \\
T1--T6 & Bias & [-0.707 , 0.039] & [0.037 , 0.215] & [-0.334 , -0.014] & [0.604 , 1.976] & [-0.122 , 0.018] & [-0.175 , 0.151] \\
T1--T6 & RMSE & [0.233 , 0.939] & [0.057 , 0.228] & [0.055 , 0.342] & [0.665 , 1.983] & [0.024 , 0.125] & [0.037 , 0.177] \\
T1--T6 & Coverage & [0.920 , 1.000] & [0.660 , 1.000] & [0.380 , 1.000] & [0.000 , 0.940] & [0.000 , 1.000] & [0.180 , 1.000] \\
\addlinespace[3pt]
\bottomrule
\end{tabular*}
\endgroup
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%% tab_n_80_200 - table 2
\begin{table}[H]
\centering
\caption{Out-of-sample predictive error summaries (CV–MSE) by MI method for $\boldsymbol{n=80}$ (left) and $\boldsymbol{n=200}$ (right), stratified by model (OLS for clean data; elastic net (EN) for contaminated data) and by missingness blocks (low: $P_{\text{miss}}\in\{0.05,0.10\}$; and high: $P_{\text{miss}}\in\{0.25,0.30\}$). For each method it is reported the min-max of the MSE: mean $\overline{X}$, variance $\sigma^2$, and median $Q_{50}$ across the corresponding design cells. Ranges further aggregate over all design combinations $P_{\text{ext}}\in\{0.03,0.05,0.10,0.15,0.30\}$, $\text{n.sim}\in\{50,300,1000\}$, $\text{iter}\in\{5,10\}$, and $\rho\in\{0,0.6\}$}
\label{tab:resumo_80_200_2}
\begingroup
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l c c c c c c @{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{n = 80}} & \multicolumn{3}{c}{\textbf{n = 200}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
MI & $\overline{X}$ & $\sigma^2$ & $Q_{50}$ & $\overline{X}$ & $\sigma^2$ & $Q_{50}$ \\
\midrule
\multicolumn{7}{l}{\textbf{Linear regression (OLS):} low missing-data proportion (5\% and 10\%)} \\
T1 & [2.397 , 2.493] & [0.009 , 0.019] & [2.403 , 2.490] & [1.983 , 2.089] & [0.003 , 0.007] & [2.000 , 2.103] \\
T2 & [2.536 , 2.580] & [0.010 , 0.023] & [2.537 , 2.583] & [2.141 , 2.159] & [0.004 , 0.008] & [2.144 , 2.175] \\
T3 & [2.523 , 2.568] & [0.010 , 0.021] & [2.518 , 2.576] & [2.146 , 2.161] & [0.004 , 0.009] & [2.155 , 2.169] \\
T4 & [2.534 , 2.585] & [0.009 , 0.019] & [2.522 , 2.584] & [2.142 , 2.164] & [0.003 , 0.010] & [2.144 , 2.180] \\
T5 & [2.589 , 2.673] & [0.013 , 0.030] & [2.569 , 2.660] & [2.198 , 2.284] & [0.005 , 0.016] & [2.196 , 2.302] \\
T6 & [2.522 , 2.580] & [0.009 , 0.020] & [2.509 , 2.574] & [2.144 , 2.156] & [0.004 , 0.009] & [2.144 , 2.160] \\
\addlinespace[4pt]
\cmidrule(lr){1-7}
\multicolumn{7}{l}{\textbf{Linear regression (OLS):} high missing-data proportion (25\% and 30\%)} \\
T1 & [2.093 , 2.189] & [0.036 , 0.047] & [2.095 , 2.191] & [1.628 , 1.707] & [0.015 , 0.017] & [1.624 , 1.707] \\
T2 & [2.551 , 2.600] & [0.046 , 0.056] & [2.537 , 2.601] & [2.131 , 2.170] & [0.020 , 0.024] & [2.140 , 2.185] \\
T3 & [2.499 , 2.540] & [0.045 , 0.064] & [2.514 , 2.561] & [2.132 , 2.162] & [0.021 , 0.027] & [2.092 , 2.140] \\
T4 & [2.598 , 2.652] & [0.049 , 0.065] & [2.582 , 2.659] & [2.168 , 2.203] & [0.023 , 0.029] & [2.143 , 2.184] \\
T5 & [2.811 , 2.905] & [0.049 , 0.074] & [2.807 , 2.941] & [2.433 , 2.648] & [0.021 , 0.042] & [2.427 , 2.621] \\
T6 & [2.552 , 2.600] & [0.043 , 0.059] & [2.547 , 2.669] & [2.125 , 2.189] & [0.024 , 0.032] & [2.102 , 2.176] \\
\addlinespace[4pt]
\cmidrule(lr){1-7}
\multicolumn{7}{l}{\textbf{Sparse regression (EN)}: low missing-data proportion (5\% and 10\%)} \\
T1 & [1.141 , 1.919] & [0.006 , 0.013] & [1.140 , 1.912] & [1.856 , 2.129] & [0.002 , 0.010] & [1.867 , 2.128] \\
T2 & [1.249 , 2.002] & [0.006 , 0.017] & [1.250 , 2.002] & [1.999 , 2.194] & [0.002 , 0.011] & [1.998 , 2.219] \\
T3 & [1.231 , 1.979] & [0.006 , 0.015] & [1.234 , 1.983] & [1.991 , 2.192] & [0.002 , 0.011] & [1.995 , 2.198] \\
T4 & [1.246 , 2.058] & [0.007 , 0.024] & [1.247 , 2.041] & [2.004 , 2.203] & [0.002 , 0.011] & [2.005 , 2.201] \\
T5 & [1.363 , 2.206] & [0.012 , 0.034] & [1.343 , 2.192] & [2.014 , 2.252] & [0.003 , 0.014] & [2.012 , 2.254] \\
T6 & [1.240 , 2.035] & [0.008 , 0.015] & [1.238 , 2.008] & [2.008 , 2.202] & [0.002 , 0.013] & [2.006 , 2.203] \\
\addlinespace[4pt]
\cmidrule(lr){1-7}
\multicolumn{7}{l}{\textbf{Sparse regression (EN)}: high missing-data proportion (25\% and 30\%)} \\
T1 & [1.369 , 1.578] & [0.023 , 0.033] & [1.381 , 1.586] & [1.536 , 1.761] & [0.017 , 0.022] & [1.531 , 1.763] \\
T2 & [1.726 , 2.047] & [0.040 , 0.059] & [1.751 , 2.038] & [2.017 , 2.217] & [0.024 , 0.034] & [1.994 , 2.216] \\
T3 & [1.679 , 2.010] & [0.035 , 0.048] & [1.689 , 2.007] & [2.001 , 2.193] & [0.025 , 0.029] & [1.981 , 2.201] \\
T4 & [1.772 , 2.237] & [0.044 , 0.088] & [1.767 , 2.240] & [2.047 , 2.287] & [0.024 , 0.043] & [2.034 , 2.275] \\
T5 & [2.080 , 2.639] & [0.058 , 0.116] & [2.075 , 2.680] & [2.190 , 2.506] & [0.022 , 0.049] & [2.180 , 2.504] \\
T6 & [1.716 , 2.149] & [0.036 , 0.099] & [1.732 , 2.137] & [2.059 , 2.251] & [0.030 , 0.034] & [2.065 , 2.265] \\
\addlinespace[4pt]
\bottomrule
\end{tabular*}
\endgroup
\end{table}
